RKHS-SHAP: Shapley Values for Kernel Methods

Feature attribution for kernel methods is often heuristic and not individualised for each prediction. To address this, we turn to the concept of Shapley values~(SV), a coalition game theoretical framework that has previously been applied to different machine learning model interpretation tasks, such as linear models, tree ensembles and deep networks. By analysing SVs from a functional perspective, we propose \textsc{RKHS-SHAP}, an attribution method for kernel machines that can efficiently compute both \emph{Interventional} and \emph{Observational Shapley values} using kernel mean embeddings of distributions. We show theoretically that our method is robust with respect to local perturbations - a key yet often overlooked desideratum for consistent model interpretation. Further, we propose \emph{Shapley regulariser}, applicable to a general empirical risk minimisation framework, allowing learning while controlling the level of specific feature's contributions to the model. We demonstrate that the Shapley regulariser enables learning which is robust to covariate shift of a given feature and fair learning which controls the SVs of sensitive features.

==> sections/05-experiments_depreciated_.tex <==
% \section{Applications and Experiments}


% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.66\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/ShapleyBanana/New_banana_experiments.pdf}
%          %\caption{\centering{Estimating Interventional and Observational Shapley values \\ using the Banana distribution dataset}}
%          \caption{\textsc{RKHS-SHAP} experiments}
%          \label{fig:y equals x}
%      \end{subfigure}%
%      \begin{subfigure}[b]{0.33\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/Defend_Robust.pdf}
%         %  \caption{\textsc{ISV-Reg}: RMSEs of  $f_{\text{reg}}$ on noisy test data at different noise level $\sigma'$.}
%         \caption{\textsc{ISV-Reg} experiments}
%          \label{fig:five over x}
%      \end{subfigure}%
%         \caption{(a) \textsc{RKHS-SHAP}: Estimation of Shapley values using data from the Banana distribution. Run time analysis is also reported. (b) \textsc{ISV-Reg}: RMSEs of $f_{\text{reg}}$ on noisy test data at different noise level $\sigma'$. All scores are averaged over 10 runs and 1 sd is reported.}
%         \label{fig:three graphs}
% \end{figure*}

% We evaluate and demonstrate both \textsc{RKHS-SHAP} and the Shapley regularisers on synthetic experiments. In the following, we denote \textsc{rkhs-osv} and \textsc{rkhs-isv} as OSVs and ISVs obtained using the \textsc{RKHS-SHAP} algorithm. We also implement the model agnostic sampling based algorithm \textsc{KernelSHAP} from the Python package \textbf{shap}\footnote{https://github.com/slundberg/shap} as a benchmark. We denote the ISV obtained from \textsc{KernelSHAP} as \textsc{kshap-isv}. As \textbf{shap} does not offer model-agnostic OSVs algorithm, we implemented the \cite{aas2019explaining}'s approach as described in Section 3, where OSVs are estimated using Monte Carlo samples from a fitted multivariate Gaussian. We call this approach \textsc{gshap-osv}. Throughout the experiments, we will use kernel ridge regression (KRR) with product RBF kernel as our model $f$. Lengthscales of the kernel is picked using median heuristic \citep{flaxman2016bayesian} and regularisation parameters $\lambda_f$ using cross-validation.

% \subsection{Estimating OSVs from the Banana distribution $\cB(b, v)$}
% We consider the following $2d$ Banana distribution \citep{sejdinovic2014kernel}: We first sample from $Z\sim \cN(0, \operatorname{diag}(v, 1))$ and transform the data by setting $X_1 = Z_1$ and $X_2 = b(Z_1^2 - v) + Z_2$ and define $f_{\text{truth}}(x) = b(x_1^2 - v) + x_2$. This formulation allows us to compute the true OSVs in closed form, i.e $\phi_{x, 1}(f_{\text{truth}}) = \frac{1}{2}(3b(x_1^2 - v) - x_2)$ and $\phi_{x, 2}(f_{\text{truth}}) = \frac{1}{2}(3x_2 - b(x_1^2 -v))$, while providing conditional densities $p(x_1|x_2)$ and $p(x_2|x_1)$ that are challenging to estimate. See Figure \ref{fig: shapley banana}a for visualisations of $X_1$ and $X_2$ at different $b$s. The higher $b$ is, the more twisted the banana shape is, making the conditional densities more difficult to estimate. 

% \textbf{Accuracy in estimating OSVs}\quad In the first experiment, we sample $1000$ points from $\cB(b, 10)$ with $b\in [0.01, 0.1, 10, 100]$ and pass it through the function $f_{\text{truth}}$ to obtain our regression labels. After fitting the kernel ridge regression, we obtain 4 sets of Shapley values from $\textsc{rkhs-isv}, \textsc{rkhs-osv}$ and $\textsc{kshap-isv}$ and $\textsc{gshap-osv}$. Figure \ref{fig: shapley banana}b illustrates ratios of RMSEs of all methods with respect to $\textsc{rkhs-osv}$. Further experiment results such as the raw RMSEs are presented in the supplementary material. We see that as $b$ increases, which indicates increases in correlation between the two features, performance in $\textsc{rkhs-isv}$ and $\textsc{kshap-isv}$ drop, as they both assumed feature independence.  As $b$ increases, we also see that $\textsc{gshap-osv}$ is performing worse because the conditional distributions $p(X_1|X_2)$ and $p(X_2|X_1)$ are further away from being multivariate Gaussians. In conclusion, $\textsc{RKHS-OSV}$ outperformed the rest, even when features are almost independent at small values of $b$, showcasing the flexibility of our method.

% \textbf{Run time analysis }\quad In this experiment we sample $n$ data points from $\cB(100, 0.1)$ where $n\in [100, 500, 1000, 1500, 3000, 5000]$ and record the $\log_{10}$ seconds required to complete the algorithm. In practice, as the software documentation of \textbf{shap} suggests, one is encouraged to summarise their dataset first using \textsc{KMeans} clustering before passing to \textsc{KernelSHAP} algorithm as the background sampling distribution. This improves computational performance significantly but at the expense of estimation accuracy as less data is used. For fair comparison with our $\textsc{RKHS-SHAP}$ methods which utilise the full training set, we also use the full training set as the background distribution for the \textsc{KernelSHAP} algorithm. Figure \ref{fig: shapley banana}c illustrated the run time across methods. We note that the difference in runtime between \textsc{KSHAP-ISV} and \textsc{GSHAP-OSV} can be attributed to a different software implementation, but we can observe that they are both significantly slower than our proposed RKHS-based Shapley value computations. Running CME based $\textsc{RKHS-OSV}$ is slower than $\textsc{RKHS-ISV}$ as estimating CMEs requires matrix inversion. In practice one could incorporate kernel approximation techniques such as Random Fourier Features to speed up kernel computation as mentioned in Section 2.

% \subsection{Regularisation experiments}
% For the following two experiments we will simulate $1000$ data from $X \sim \cN(0, \Sigma)$ with $\operatorname{diag}(\Sigma)=\mathbf{1}_5$, $\Sigma_{4,5} = \Sigma_{5,4} = 0.9$ and 0 otherwise. This indicates strong correlation between features 4 and 5 and independence otherwise. We set our label as $y = X^\top \beta$ with $\beta = [1, 2, 3, 4, 15]$, enforcing the $5^{th}$ feature to be the most influential one. As standard regression practice, we do a $70-30$ train-test split on the data.

% \textbf{Protection against covariate shift using \textsc{ISV-Reg}}\quad In this experiment, we inject extra mean zero Gaussian noise to the $5^{th}$ feature in the testing set, i.e $X_5' = X_5 + \sigma'\cN(0, 1)$ for $\sigma' \in [0, 0.1, 0.5, 1, 1.5]$. Knowing there will be covariate shift at test time, which could happen in real world for example due to instrumental uncertainty, we train our kernel ridge regression $f_{\text{reg}}$ with \textsc{ISV-Reg} at different regularisation level $\lambda_{SV}$ for $\lambda_{SV}\in [0, 0.5, 1, 1.5, 2, 2.5]$. We then compare RMSEs between labels predicted using the noisy data and labels predicted using noiseless ground-truth data ($\sigma'=0$). Figure \ref{fig: robustness} illustrates such RMSEs across different configurations of regularisation and data noise. We see when no regularisation is applied, the RMSE spikes up as $\sigma'$ increases, indicating our standard kernel ridge regressor is sensitive to noises from $X_5$. As regularisation increases, we \emph{significantly} reduce the RMSEs from noisy data, at the price of increasing RMSE at noiseless data gradually.

% \textbf{Applying \textsc{OSV-Reg} for fair learning}\quad
% Here we treat feature $X_5$ as the sensitive feature and minimise its contribution to our model $f_{\text{reg}}$ by running \textsc{OSV-reg} at various regularisation parameter $\lambda_{SV}$. We also implement $\textsc{ISV-reg}$ to emphasis the importance of taking correlation into account during regularisation for fair learning. Figure \ref{fig: everyone-reg} shows that as $\lambda_{SV}$ increases, which corresponds to color intensities of the line, the more the distributions of $\phi_{X, 5}^{(I)}(f_{\text{reg}})$ and $\phi_{X, 5}^{(O)}(f_{\text{reg}})$ are peaked around 0, indicating lesser contribution to the  learning. However, regarding the highly correlated variable $X_4$, while the $\phi_{X, 4}^{(O)}(f_{\text{reg}})$ exhibits a similar behavior as $\phi_{X, 5}^{(O)}(f_{\text{reg}})$, $\phi_{X, 4}^{(I)}(f_{\text{reg}})$ remains fairly evenly distributed, meaning that $\textsc{ISV-Reg}$ cannot handle the omitted variable biases during learning.

% % the more centred $\phi_{X, 5}^{(I)}(f_{\text{reg}})$ and $\phi_{X, 5}^{(O)}(f_{\text{reg}})$ distribute, indicating $X_5$ contributes less and less to the model. However, regarding the highly correlated variable $X_4$, while the $\phi_{X, 4}^{(O)}(f_{\text{reg}})$ exhibits a similar behavior as $\phi_{X, 5}^{(O)}(f_{\text{reg}})$, $\phi_{X, 4}^{(I)}(f_{\text{reg}})$ remains fairly evenly distributed, meaning that $\textsc{ISV-Reg}$ cannot handle the omitted variable biases during learning.

% % \begin{figure}[]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figure/Defend_Robust.pdf}
% %     \caption{\textsc{ISV-Reg}: RMSEs of regularised $f_{\text{reg}}$ on noisy test data with different noise level $\sigma'$. }
% %     \label{fig: robustness}
% % \end{figure}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/reg_trend.pdf}
%     \caption{Distributions of ISVs and OSVs of sensitive feature $X_5$ and its strongly correlated feature $X_4$ obtained from $\textsc{ISV-Reg}$ and $\textsc{OSV-Reg}$ at different regularisation parameters. Intensity of colour represents the strength of regularisation. The more peaked the distribution of SVs is, the less it contributes to the learning. }
%     \label{fig: everyone-reg}
% \end{figure}


